Part-wise Certified State Estimation of Articulated Objects from Passive Stereo

Robots in manufacturing often handle thin, hinged objects known from CAD models that change shape during the task, like folding cartons. Monitoring such tasks requires estimating the object's articulation state, its pose and the shape of any semi-deformable part. Learning-based estimators generalise across objects but lose precision while handling thin parts. Model-based fitting is precise but often needs accurate depth, a close initial estimate and a clean object mask. We present part-wise certification of an articulated object's state, estimated from passive stereo. Our estimator rivals the precision of the best model-based fitting method without using depth, a close initial estimate or a mask. We detect the corners that the CAD model defines in both stereo images and fit the articulated model to them. Geometric certificates, which we extend from rigid to articulated objects, then tell whether to trust each part, because the fit returns a state even for hidden parts. Certified estimates on unlabelled video become labels that improve sim-to-real transfer. On five of seven simulated objects, we locate the parts we certify three to five times more precisely than the strongest learned baseline on the same readings, given depth and true masks. On a real folding carton, our median corner error on the end panels is 2.1% of the carton's size, at least 40% lower than every learned baseline and also lower than a depth-based fit initialised near the true state.

==> figs/pipe/tile_coords.tex <==
\def\zAxa{0.5856}%
\def\zAya{0.4821}%
\def\zAxb{1.0056}%
\def\zAyb{0.9021}%
\def\zBx{0.8133}%
\def\zBy{0.3456}%
\def\zBr{0.1463}%
\def\zFxa{0.5056}%
\def\zFya{0.3940}%
\def\zFxb{1.0000}%
\def\zFyb{0.8883}%

